Maat: Performance Metric Anomaly Anticipation for Cloud Services with Conditional Diffusion

Ensuring the reliability and user satisfaction of cloud services necessitates prompt anomaly detection followed by diagnosis. Existing techniques for anomaly detection focus solely on real-time detection, meaning that anomaly alerts are issued as soon as anomalies occur. However, anomalies can propagate and escalate into failures, making faster-than-real-time anomaly detection highly desirable for expediting downstream analysis and intervention. This paper proposes Maat, the first work to address anomaly anticipation of performance metrics in cloud services. Maat adopts a novel two-stage paradigm for anomaly anticipation, consisting of metric forecasting and anomaly detection on forecasts. The metric forecasting stage employs a conditional denoising diffusion model to enable multi-step forecasting in an auto-regressive manner. The detection stage extracts anomaly-indicating features based on domain knowledge and applies isolation forest with incremental learning to detect upcoming anomalies. Thus, our method can uncover anomalies that better conform to human expertise. Evaluation on three publicly available datasets demonstrates that Maat can anticipate anomalies faster than real-time comparatively or more effectively compared with state-of-the-art real-time anomaly detectors. We also present cases highlighting Maat's success in forecasting abnormal metrics and discovering anomalies.

==> algo-tables/table-baselines.tex <==
\begin{table}[htb]
\vspace{-0.1in}
\small
\centering
\caption{Compared approaches of \tool.}
\vspace{-0.1in}
\begin{tabular}{cccc}
\toprule
Approach & Variate & Supervised? & Core Technique  \\
\midrule
Dount~\cite{dount} & Uni- & No & VAE \\
SR-CNN~\cite{srcnn} & Uni- &  No & CNN \\
Adsketch~\cite{adsketch} & Uni- & Semi- & pattern sketching \\
Telemanom~\cite{telemanom} & Multi- & No & LSTM \\
LSTM-VAE~\cite{lstm-vae} & Multi- & No & LSTM \& VAE \\
MTAD-GAT~\cite{mtad} & Multi- & No & GAT \\
DAGMM~\cite{dagmm} &  Multi- & No & AE \& Gaussian Mixture \\
OmniAnomaly~\cite{OmniAnomaly} & Multi- & No & RNN \& VAE \\
\bottomrule
\end{tabular}\label{tab:baselines}
\vspace{-0.1in}
\end{table}

%They are Dount~\cite{dount}, SR-CNN~\cite{srcnn}, Adsketch~\cite{adsketch}, Telemanom~\cite{telemanom}, LSTM-VAE~\cite{lstm-vae}, MTAD-GAT~\cite{mtad}, DAGMM~\cite{dagmm}, and OmniAnomaly~\cite{OmniAnomaly}.
% \begin{itemize}
%     \item Dount~\cite{dount} is an unsupervised anomaly detection algorithm for univariate metrics based on Variational Autoencoder (VAE). It compares the reconstructed metrics and the really observed metrics and alerts anomalies when obtaining a large reconstruction loss.
%     \item SR-CNN~\cite{srcnn} applies residual spectrum (SR) from the visual saliency detection domain to time series anomaly detection. The SR model generates pseudo labels to train the subsequent convolutional neural network, which will output a binary result to indicate anomalies.
%     \item Adsketch~\cite{adsketch} is a recently proposed method that adaptively detects performance anomalies based on pattern sketching. It is semi-supervised in a sense as it requires anomaly-free inputs to extract normal patterns. If the current metric patterns are not similar to previous patterns, an alarm will be triggered.
%     \item Telemanom~\cite{telemanom} combines long-short-term-memory (LSTM) with an auto-thresholding algorithm. The trained LSTM first predicts the next-time metric, and if the prediction error is larger than the automatically decided threshold, Telemanom will report an anomaly.
%     \item LSTM-VAE~\cite{lstm-vae} also works by reconstructing subsequences of metrics, similar to Dount. It combines LSTM with VAE and can handle multivariate time series.
%     \item MTAD-GAT~\cite{mtad} combines both prediction-based approaches (e.g., Telemanom) and reconstruction-based approaches (e.g., Dount). It considers every single metric as a feature and then uses two parallel graph attention network (GAT) layers to learn the temporal and cross-metric dependencies. The two models will jointly output an inference score as the basis of anomaly detection.
%     \item DAGMM~\cite{dagmm} combines a deep autoencoder and a Gaussian Mixture Model to estimate the anomaly score of each to-be-detected metric subsequence.
%     \item OmniAnomaly~\cite{OmniAnomaly} is a stochastic recurrent neural network for multivariate time series anomaly detection based on VAE. It aims to learn potential representations to capture normal patterns of metrics while considering time dependencies and stochasticity.
% \end{itemize}


